Multi-Frame Self-Supervised Depth with Transformers

Multi-frame depth estimation improves over single-frame approaches by also leveraging geometric relationships between images via feature matching, in addition to learning appearance-based features. In this paper we revisit feature matching for self-supervised monocular depth estimation, and propose a novel transformer architecture for cost volume generation. We use depth-discretized epipolar sampling to select matching candidates, and refine predictions through a series of self- and cross-attention layers. These layers sharpen the matching probability between pixel features, improving over standard similarity metrics prone to ambiguities and local minima. The refined cost volume is decoded into depth estimates, and the whole pipeline is trained end-to-end from videos using only a photometric objective. Experiments on the KITTI and DDAD datasets show that our DepthFormer architecture establishes a new state of the art in self-supervised monocular depth estimation, and is even competitive with highly specialized supervised single-frame architectures. We also show that our learned cross-attention network yields representations transferable across datasets, increasing the effectiveness of pre-training strategies. Project page: https://sites.google.com/tri.global/depthformer

==> figures/cal.tex <==

\begin{figure}[t!]
    \centering
    \subfloat{
    \includegraphics[width=0.16\textwidth,height=1.3cm]{media/figures/ddad/val-ddad-val-lidar-cam1-768-rgb(0)_50_fb72f33f.png}}
    \subfloat{
    \includegraphics[width=0.16\textwidth,height=1.3cm]{media/figures/ddad/val-ddad-val-lidar-cam1-768-pred-depth_regr_mask_debug(0)_0_50_70bec55e.png}}
    \subfloat{
    \includegraphics[width=0.16\textwidth,height=1.3cm]{media/figures/ddad/val-ddad-val-lidar-cam1-768-pred-depth_multi(0)_0_50_fa3163c9.png}}
    \\ \vspace{-3mm}
    \setcounter{subfigure}{0}
    \subfloat[Input target image]{
    \includegraphics[width=0.16\textwidth,height=1.3cm]{media/figures/ddad/val-ddad-val-lidar-cam1-1536-rgb(0)_50_c371621a.png}}
    \subfloat[High-response depth]{
    \includegraphics[width=0.16\textwidth,height=1.3cm]{media/figures/ddad/val-ddad-val-lidar-cam1-1536-pred-depth_regr_mask_debug(0)_0_50_a457fa92.png}}
    \subfloat[Context-adjusted depth]{
    \includegraphics[width=0.16\textwidth,height=1.3cm]{media/figures/ddad/val-ddad-val-lidar-cam1-1536-pred-depth_multi(0)_0_50_09e73c20.png}}
    \\    
    \label{fig:cal}
    \caption{
    \textbf{Context-adjusted depth} results for KITTI.
}
\end{figure}

==> figures/confidence.tex <==

\begin{figure}[t!]
    % \vspace{-5mm}
    \centering
    \subfloat[Input image]{
        \includegraphics[width=0.15\textwidth]{media/figures/confidence/val-ddad-val-lidar-cam1-768-rgb(0)_37_fb72f33f.png}
    }
    \subfloat[Maximum attention]{
        \includegraphics[width=0.15\textwidth]{media/figures/confidence/val-ddad-val-lidar-cam1-768-mask_norm_31_3808206c_B.png}
        \label{fig:max_attention}
    }    
    \subfloat[High-response depth]{
        \includegraphics[width=0.15\textwidth]{media/figures/confidence/val-ddad-val-lidar-cam1-768-pred-depth_regr_mask_debug(0)_0_37_380e3576.png}
        \label{fig:high_response_depth}
    }
    \caption{\textbf{Example of high-response depth estimation.} Maximum normalized attention values decrease with distance, and can be used as a measure of confidence for pixel masking.
    }
    \label{fig:confidence}
\end{figure}

==> figures/decoded_depth.tex <==

\begin{figure*}[t!]
    \label{fig:decoded_depth}
    \centering
    \subfloat{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/rgb_50.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/match_50.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/mask_50.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/depth_50.png}}
    \\
    \setcounter{figure}{0}
    \subfloat[Current frame]{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/rgb_54.png}}
    \subfloat[SSIM depth]{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/match_54.png}}
    \subfloat[Cost-attention depth]{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/mask_54.png}}
    \subfloat[Decoded depth]{
    \includegraphics[width=0.24\textwidth]{media/figures/decoders/depth_54.png}}
    \caption{
        \textbf{Qualitative results} our different .
}
\end{figure*}

==> figures/high_response.tex <==

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4\textwidth]{media/figures/high_response2.png}
    \caption{
        \textbf{High response depth estimation} from a cross-attention cost volume. Instead of a weighted sum of all candidates, we use a window centered on the most probable candidate. 
    }
    \label{fig:high_response}
\end{figure}

==> figures/qualitative.tex <==

\begin{figure*}[t!]
    \centering
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000023(0)_rgb.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000023_depth_regr_mask_debug(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000023_depth_regr(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000023_depth_multi(0)_pred_viz.png}}
    \\
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000024(0)_rgb.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000024_depth_regr_mask_debug(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000024_depth_regr(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000024_depth_multi(0)_pred_viz.png}}
    \\
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000036(0)_rgb.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000036_depth_regr_mask_debug(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000036_depth_regr(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000036_depth_multi(0)_pred_viz.png}}
    \\
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000049(0)_rgb.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000049_depth_regr_mask_debug(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000049_depth_regr(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000049_depth_multi(0)_pred_viz.png}}
    \\
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000056(0)_rgb.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000056_depth_regr_mask_debug(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000056_depth_regr(0)_pred_viz.png}}
    \subfloat{
    \includegraphics[width=0.24\textwidth,height=1.3cm]{media/figures/qualitative/0000000056_depth_multi(0)_pred_viz.png}}
    \\    
    \caption{
}
\label{fig:qualitative}
\end{figure*}

==> figures/teaser.tex <==


\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\textwidth,height=3cm]{media/figures/teaser_two.png}
    \caption{
    \textbf{Our DepthFormer architecture} achieves state-of-the-art multi-frame self-supervised monocular depth estimation by \textbf{improving feature matching} during cost volume generation.
    }
    \label{fig:teaser}
\vspace{-5mm}
\end{figure*} 

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.4\textwidth,height=7.5cm]{media/figures/teaser/teaser4.png}
%     \caption{
%     \textbf{Our DepthFormer architecture} achieves state-of-the-art multi-frame self-supervised monocular depth estimation by \textbf{improving feature matching} during cost volume generation.
%     }
%     \label{fig:teaser}
% \vspace{-5mm}
% \end{figure} 

==> tables/kitti_depth.tex <==
\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
% \renewcommand{\arraystretch}{0.95}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|l|c|c|c|c|cccc|ccc}
\toprule
&
\multirow{2}[2]{*}{\textbf{Method}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Superv.}}} &
\multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Multi-Fr.}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Synthetic}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Semantic}}} & 
\multicolumn{4}{c|}{\textit{Lower is better}} &
\multicolumn{3}{c}{\textit{Higher is better}} 
\\
\cmidrule(lr){7-10} \cmidrule(lr){11-13}
& & & & & &
AbsRel &
SqRel &
RMSE &
RMSE$_{log}$ &
$\delta < {1.25}$ &
$\delta < {1.25}^2$ &
$\delta < {1.25}^3$
\\
\midrule
\parbox[t]{2mm}{\multirow{14}{*}{\rotatebox[origin=c]{90}{Original~\cite{eigen2014depth}}}}
& Ranjan \emph{et al.} \cite{competi_colab}
& M & & & 
& 0.148 & 1.149 & 5.464 & 0.226 & 0.815 & 0.935 & 0.973 
\\
& EPC++ \cite{epc++}
& M & & & 
& 0.141 & 1.029 & 5.350 & 0.216 & 0.816 & 0.941 & 0.976 
\\
& Struct2Depth \cite{casser2018depth}
& M & & & \checkmark
& 0.141 & 1.026 & 5.291 & 0.215 & 0.816 & 0.945 & 0.979 
\\
& Li \emph{et al.} \cite{dynamic_scenes}
& M & & & 
& 0.130 & 0.950 & 5.138 & 0.209 & 0.843 & 0.948 & 0.978 
\\
& Gordon \emph{et al.} \cite{gordon2019depth}
& M & & & \checkmark
& 0.128 & 0.959 & 5.230 & 0.212 & 0.845 & 0.947 & 0.976 
\\
& GASDA \cite{gasda}
& M & & \checkmark &
& 0.120 & 1.022 & 5.162 & 0.215 & 0.848 & 0.944 & 0.974
\\
& SharinGAN \cite{sharingan}
& M & & \checkmark &
& 0.116 & 0.939 & 5.068 & 0.203 & 0.850 & 0.948 & 0.978
\\
& Monodepth2 \cite{monodepth2}
& M & & & 
& 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981 
\\
& Patil \emph{et al.} \cite{forget_past}
& M & \checkmark & & 
& 0.111 & 0.821 & 4.650 & 0.187 & 0.883 & 0.961 & 0.982 
\\
& PackNet-SFM \cite{packnet}
& M & & & 
& 0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982 
\\
& Johnston \emph{et al.} \cite{johnston2020selfsupervised}
& M & & & 
& 0.106 & 0.861 & 4.699 & 0.185 & 0.889 & 0.962 & 0.982 
\\
& Wang \emph{et al.} \cite{implicit_cues}
& M & \checkmark & & 
& 0.106 & 0.799 & 4.662 & 0.187 & 0.889 & 0.961 & 0.982 
\\
& MonoDEVSNet \cite{virtualworld}
& M & & \checkmark &
& 0.104 & 0.721 & 4.396 & 0.185 & 0.880 & 0.962 & \underline{0.983}
\\
& Guizilini \emph{et al.} \cite{packnet-semguided}
& M & & & \checkmark
& 0.102 & \underline{0.698} & \underline{4.381} & 0.178 & 0.896 & 0.964 & \textbf{0.984} 
\\
& ManyDepth \cite{manydepth} 
& M & \checkmark & & 
& \underline{0.098} & 0.770 & 4.459 & \underline{0.176} & \underline{0.900} & \underline{0.965} & \underline{0.983} 
\\
\cmidrule{2-13}
& \textbf{DepthFormer} 
& M & \checkmark & & 
% & \textbf{0.094} & \underline{0.712} & \textbf{4.243} & \underline{0.177} & \textbf{0.900} & \textbf{0.966} & \textbf{0.985} 
& \textbf{0.090} & \textbf{0.661} & \textbf{4.149} & \textbf{0.175} & \textbf{0.905} & \textbf{0.967} & \textbf{0.984} 
\\
\midrule
\midrule
\parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Improved~\cite{gtkitti}}}}
& Kuznietsov \emph{et al.} \cite{kuznietsov2017semi}
& D & & & 
& 0.113 & 0.741 & 4.621 & 0.189 & 0.862 & 0.960 & 0.986 
\\
& Gan \emph{et al.} \cite{Gan2018MonocularDE}
& D & & & 
& 0.098 & 0.666 & 3.933 & 0.173 & 0.890 & 0.964 & 0.985 
\\
& Guizilini \emph{et al.} \cite{packnet-semisup}
& D & & & 
& 0.072 & 0.340 & 3.265 & 0.116 & 0.934 & --- & --- 
\\
& DORN \cite{fu2018deep} 
& D & & & 
& 0.072 & 0.307 & \textbf{2.727} & 0.120 & 0.932 & 0.984 & 0.994 
\\
& Yin \emph{et al.} \cite{Yin2019enforcing}
& D & & & 
& 0.072 & --- & 3.258 & 0.117 & 0.938 & 0.990 & \textbf{0.998} 
\\
& PackNet-SFM \cite{packnet}
& M & & & 
& 0.078 & 0.420 & 3.485 & 0.121 & 0.931 & 0.986 & 0.996 
\\
& ManyDepth \cite{manydepth} 
& M & \checkmark & & 
& 0.064 & 0.320 & 3.187 & 0.104 & 0.946 & 0.990 & 0.995 
\\
& BTS \cite{lee2019big} 
& D & & & 
& \underline{0.059} & \textbf{0.245} & \underline{2.756} & \underline{0.096} & \textbf{0.956} & \textbf{0.993} & \textbf{0.998} 
\\
% & MonoREC \cite{monorec} 
% & MS+D$^*$ & & & & 
% & 0.050 & 0.295 & 2.266 & 0.082 & 0.973 & 0.991 & 0.996 
% \\
% & TransDepth \cite{yang2021transformers} 
% & D & & & & 
% & 0.064 & 0.252 & 2.755 & 0.098 & 0.956 & 0.994 & 0.999 
% \\
% & DPT \cite{yang2021transformers} 
% & D & & & & 
% & 0.062 & --- & 2.573 & 0.092 & 0.959 & 0.995 & 0.999 
% \\
\cmidrule{2-13}
& \textbf{DepthFormer} 
& M & \checkmark & & 
% & \textbf{0.059} & \underline{0.302} & 3.032 & \underline{0.099} & \underline{0.949} & \underline{0.990} & \underline{0.997} 
& \textbf{0.055} & \underline{0.271} & 2.917 & \textbf{0.095} & \underline{0.955} & \underline{0.991} & \textbf{0.998} 
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Depth results} on the KITTI \emph{Eigen} test split \cite{eigen2014depth}, for distances up to 80m with the \emph{Garg} crop, evaluated on the two available ground-truth depth maps~\cite{eigen2014depth,gtkitti}. \emph{Superv.} indicates the source of supervision (M for monocular self-supervision and D for depth supervision); \emph{Multi-Fr.} the use of multiple frames at test time; \emph{Synthetic} the use of synthetic data; and \emph{Semantic} the use of additional semantic information. 
}
\label{table:kitti_depth}
% \vspace{-5mm}
\end{table*}


==> tables/performance.tex <==

\captionsetup[table]{skip=6pt}

\begin{table}[t!]
\small
% \renewcommand{\arraystretch}{0.95}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|c|c||cc|cc}
\toprule
& \multicolumn{3}{c||}{Variation} & \multicolumn{2}{c}{GPU (GB)} & \multicolumn{2}{|c}{FPS (im/s)} 
\\
\midrule
& N & C & D & train & test & train & test 
\\
\midrule
& 6 & 128 & 128 & 
12.2 & 5.3 & --- & ---
\\
% \midrule
$\dagger$ & 6 & 128 & 128 & 
5.9 & 5.3 & --- & ---
\\
\midrule
& 4 & 128 & 128 & 
10.3 & 5.1 & --- & ---
\\
& 2 & 128 & 128 & 
8.4 & 5.0 & --- & ---
\\
\midrule
& 6 & 96 & 128 & 
9.5 & 4.4 & --- & ---
\\
& 6 & 48 & 128 & 
6.6 & 3.2 & --- & --- 
\\
& 6 & 32 & 128 & 
5.7 & 2.6 & --- & --- 
\\
\midrule
& 6 & 128 & 96 & 
10.1 & 4.4 & --- & --- 
\\
& 6 & 128 & 48 & 
6.9 & 3.3 & --- & --- 
\\
& 6 & 128 & 16 & 
5.6 & 2.4 & --- & --- 
\\
\midrule
& 2 & 32 & 16 & 
3.8 & 1.9 & --- & --- 
\\
% \midrule
$\dagger$ & 2 & 32 & 16 & 
2.9 & 1.9 & --- & --- 
\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Training time and memory requirements} for our proposed architecture. The $\dagger$ symbol indicates a frozen attention network (no fine-tuning during training). 
}
\label{table:performance2}
\end{table}

